Modeling Fine-grained Information via Knowledge-aware Hierarchical Graph for Zero-shot Entity Retrieval

Zero-shot entity retrieval, aiming to link mentions to candidate entities under the zero-shot setting, is vital for many tasks in Natural Language Processing. Most existing methods represent mentions/entities via the sentence embeddings of corresponding context from the Pre-trained Language Model. However, we argue that such coarse-grained sentence embeddings can not fully model the mentions/entities, especially when the attention scores towards mentions/entities are relatively low. In this work, we propose GER, a \textbf{G}raph enhanced \textbf{E}ntity \textbf{R}etrieval framework, to capture more fine-grained information as complementary to sentence embeddings. We extract the knowledge units from the corresponding context and then construct a mention/entity centralized graph. Hence, we can learn the fine-grained information about mention/entity by aggregating information from these knowledge units. To avoid the graph information bottleneck for the central mention/entity node, we construct a hierarchical graph and design a novel Hierarchical Graph Attention Network~(HGAN). Experimental results on popular benchmarks demonstrate that our proposed GER framework performs better than previous state-of-the-art models. The code has been available at https://github.com/wutaiqiang/GER-WSDM2023.

==> 3_formulation.tex <==
\section{Formulation}
%Introduction the formulation of entity linking and zero-shot entity linking
\paragraph{Entity Linking}
Given an unstructured text $c$ with a pre-identified mention $m$, the goal of entity linking system is to find a corresponding entity $e$ from knowledge base  $\mathcal{E} = \{e_1, e_2, \ldots, e_N\}$. The size of knowledge base $N$ can be very large such as $5.9M$ for Wikipedia, and encoding those entities is time costing.
%
To address this problem, a common strategy is considering entity linking in two-stage paradigm: (i) retrieval $k$ candidate entities $\{e^1_i, e^2_i, \ldots, e^k_i\} $ for mention $m_i$, where $k \ll N$. (ii) rank these candidate entities.

\paragraph{Zero-shot Entity Linking} Under zero-shot setting, there is no graph information but corresponding entity description $d$ for each entity $e$. Moreover, we require $\mathcal{E}_{train} \bigcap \mathcal{E}_{test} = \emptyset$ where $\mathcal{E}_{train}$ and $\mathcal{E}_{test}$ means the knowledge base for train and test. In this paper, we mainly focus on the problem of candidate retrieval stage, given the mention context $(m,c)$ and the entity description $(e,d)$.
